Platonic crystal with low-frequency locally resonant snail structures. Wave trapping, transmission amplification and shielding

We propose a new type of platonic crystal. The proposed microstructured plate includes snail resonators with low-frequency resonant vibrations. The particular dynamic effect of the resonators are highlighted by a comparative analysis of dispersion properties of homo- geneous and perforated plates. Analytical and numerical estimates of classes of standing waves are given and the analysis on a macrocell shows the possibility to obtain localization, wave trapping and edge waves. Applications include transmission amplification within two plates separated by a small ligament. Finally we proposed a design procedure to suppress low frequency flexural vibration in an elongated plate implementing a by-pass system re- routing waves within the mechanical system.

==> macro.tex <==
% Reduce space surrounding equal signs (=) in equation arrays.
\setlength{\arraycolsep}{2pt}
% Set up counter for list environments
\newcounter{itemnbr}
% Handy abbreviations.
\newcommand\eq[1] {(\ref{#1})}
\newcommand\eqp[1] {(\ref{eq:#1})}
\newcommand\defn[1] {\ref{def:#1}}
\newcommand\thm[1] {\ref{thm:#1}}
\newcommand\sect[1] {\ref{sec:#1}}
\newcommand\fig[1] {\ref{fig:#1}}
\newcommand\labeq[1] {\label{eq:#1}}
\newcommand\labdefn[1] {\label{def:#1}}
\newcommand\labthm[1] {\label{thm:#1}}
\newcommand\labsect[1] {\label{sec:#1}}
\newcommand\labfig[1] {\label{fig:#1}}
\newcommand\etal{{\it et al.}}
%\newcommand\B {\Bigg}
% Math environments
\newtheorem{definition}{Definition}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}{Corollary}[section]
%\newcommand\proof{{\it Proof:}\quad}
\newcommand\remark{{\it Remark:}\quad}
%\newcommand\qed{\ \rule[-0.2ex]{0.3em}{1.5ex}}
% De-verbose the LaTeX math environment
\newcommand{\bfm}[1]{\mbox{\boldmath ${#1}$}}
\newcommand{\nonum}{\nonumber \\}
\newcommand{\beqa}{\begin{eqnarray}}
\newcommand{\eeqa}[1]{\label{#1}\end{eqnarray}}
\newcommand{\bequ}{\begin{equation}}
\newcommand{\eequ}[1]{\label{#1}\end{equation}}
%\newcommand{\R}{\mbox{R}}
%\newcommand{\C}{\mbox{C}}
\newcommand{\Grad}{\nabla}
%\newcommand{\Div}{\nabla \cdot}
\newcommand{\Curl}{\nabla \times}
\newcommand{\mn}{{\rm min}}
\newcommand{\mx}{{\rm max}}
\newcommand{\lang}{\langle}
\newcommand{\rang}{\rangle}
\newcommand{\Md}{\partial}
\newcommand{\MP}{\bigoplus}
\newcommand{\MT}{\bigotimes}
\newcommand{\MU}{\bigcup}
\newcommand{\MI}{\bigcap}
\newcommand{\MV}{\bigvee}
\newcommand{\MW}{\bigwedge}
\newcommand{\ov}[1]{\overline{#1}}

% Abbreviate definitions of greek symbols
\newcommand{\Ga}{\alpha}
\newcommand{\Gb}{\beta}
\newcommand{\Gd}{\delta}
\newcommand{\Ge}{\epsilon}
\newcommand{\Gve}{\varepsilon}
\newcommand{\Gf}{\phi}
\newcommand{\Gvf}{\varphi}
\newcommand{\Gg}{\gamma}
\newcommand{\Gc}{\chi}
\newcommand{\Gi}{\iota}
\newcommand{\Gk}{\kappa}
\newcommand{\Gl}{\lambda}
\newcommand{\Gn}{\eta}
\newcommand{\Gm}{\mu}
\newcommand{\Gv}{\nu}
\newcommand{\Gp}{\pi}
\newcommand{\Gt}{\theta}
\newcommand{\Gvt}{\vartheta}
\newcommand{\Gr}{\rho}
\newcommand{\Gvr}{\varrho}
\newcommand{\Gs}{\sigma}
\newcommand{\Gvs}{\varsigma}
\newcommand{\Gj}{\tau}
\newcommand{\Gu}{\upsilon}
\newcommand{\Go}{\omega}
\newcommand{\Gx}{\xi}
\newcommand{\Gy}{\psi}
\newcommand{\Gz}{\zeta}
\newcommand{\GD}{\Delta}
\newcommand{\GF}{\Phi}
%\newcommand{\GG}{\Gamma}
\newcommand{\GL}{\Lambda}
\newcommand{\GP}{\Pi}
\newcommand{\GT}{\Theta}
\newcommand{\GS}{\Sigma}
\newcommand{\GU}{\Upsilon}
\newcommand{\GO}{\Omega}
\newcommand{\GX}{\Xi}
\newcommand{\GY}{\Psi}

% Abbreviate definitions of bold greek symbols: note that defs.tex is 
% needed first
\newcommand{\BGa}{\bfm\alpha}
\newcommand{\BGb}{\bfm\beta}
\newcommand{\BGd}{\bfm\delta}
\newcommand{\BGe}{\bfm\epsilon}
\newcommand{\BGve}{\bfm\varepsilon}
\newcommand{\BGf}{\bfm\phi}
\newcommand{\BGvf}{\bfm\varphi}
\newcommand{\BGg}{\bfm\gamma}
\newcommand{\BGc}{\bfm\chi}
\newcommand{\BGi}{\bfm\iota}
\newcommand{\BGk}{\bfm\kappa}
\newcommand{\BGl}{\bfm\lambda}
\newcommand{\BGn}{\bfm\eta}
\newcommand{\BGm}{\bfm\mu}
\newcommand{\BGv}{\bfm\nu}
\newcommand{\BGp}{\bfm\pi}
\newcommand{\BGt}{\bfm\theta}
\newcommand{\BGvt}{\bfm\vartheta}
\newcommand{\BGr}{\bfm\rho}
\newcommand{\BGvr}{\bfm\varrho}
\newcommand{\BGs}{\bfm\sigma}
\newcommand{\BGvs}{\bfm\varsigma}
\newcommand{\BGj}{\bfm\tau}
\newcommand{\BGu}{\bfm\upsilon}
\newcommand{\BGo}{\bfm\omega}
\newcommand{\BGx}{\bfm\xi}
\newcommand{\BMx}{\bfm\xi}
\newcommand{\BGy}{\bfm\psi}
\newcommand{\BGz}{\bfm\zeta}
\newcommand{\BGD}{\bfm\Delta}
\newcommand{\BGF}{\bfm\Phi}
\newcommand{\BGG}{\bfm\Gamma}
\newcommand{\BGL}{\bfm\Lambda}
\newcommand{\BGP}{\bfm\Pi}
\newcommand{\BGT}{\bfm\Theta}
\newcommand{\BGS}{\bfm\Sigma}
\newcommand{\BGU}{\bfm\Upsilon}
\newcommand{\BGO}{\bfm\Omega}
\newcommand{\BGX}{\bfm\Xi}
\newcommand{\BGY}{\bfm\Psi}


% Abbreviate symbols for caligraphic letters
\newcommand{\Ca}{{\cal a}}
\newcommand{\Cb}{{\cal b}}
\newcommand{\Cc}{{\cal c}}
\newcommand{\Cd}{{\cal d}}
\newcommand{\Ce}{{\cal e}}
\newcommand{\Cf}{{\cal f}}
\newcommand{\Cg}{{\cal g}}
\newcommand{\Ch}{{\cal h}}
\newcommand{\Ci}{{\cal i}}
\newcommand{\Cj}{{\cal j}}
\newcommand{\Ck}{{\cal k}}
\newcommand{\Cl}{{\cal l}}
\newcommand{\Cm}{{\cal m}}
\newcommand{\Cn}{{\cal n}}
\newcommand{\Co}{{\cal o}}
\newcommand{\Cp}{{\cal p}}
\newcommand{\Cq}{{\cal q}}
\newcommand{\Cr}{{\cal r}}
\newcommand{\Cs}{{\cal s}}
\newcommand{\Ct}{{\cal t}}
\newcommand{\Cu}{{\cal u}}
\newcommand{\Cv}{{\cal v}}
\newcommand{\Cx}{{\cal x}}
\newcommand{\Cy}{{\cal y}}
\newcommand{\Cz}{{\cal z}}
\newcommand{\CA}{{\cal A}}
\newcommand{\CB}{{\cal B}}
%\newcommand{\CC}{{\cal C}}
%\newcommand{\CD}{{\cal D}}
\newcommand{\CE}{{\cal E}}
\newcommand{\CF}{{\cal F}}
%\newcommand{\CG}{{\cal G}}
\newcommand{\CH}{{\cal H}}
\newcommand{\CI}{{\cal I}}
\newcommand{\CJ}{{\cal J}}
\newcommand{\CK}{{\cal K}}
\newcommand{\CL}{{\cal L}}
\newcommand{\CM}{{\cal M}}
\newcommand{\CN}{{\cal N}}
\newcommand{\CO}{{\cal O}}
\newcommand{\CP}{{\cal P}}
\newcommand{\CQ}{{\cal Q}}
\newcommand{\CR}{{\cal R}}
\newcommand{\CS}{{\cal S}}
\newcommand{\CT}{{\cal T}}
\newcommand{\CU}{{\cal U}}
\newcommand{\CV}{{\cal V}}
\newcommand{\CW}{{\cal W}}
\newcommand{\CX}{{\cal X}}
\newcommand{\CY}{{\cal Y}}
\newcommand{\CZ}{{\cal Z}}
% Abbreviate symbols for bold caligraphic letters
\newcommand{\BCa}{{\bfm{\cal a}}}
\newcommand{\BCb}{{\bfm{\cal b}}}
\newcommand{\BCc}{{\bfm{\cal c}}}
\newcommand{\BCd}{{\bfm{\cal d}}}
\newcommand{\BCe}{{\bfm{\cal e}}}
\newcommand{\BCf}{{\bfm{\cal f}}}
\newcommand{\BCg}{{\bfm{\cal g}}}
\newcommand{\BCh}{{\bfm{\cal h}}}
\newcommand{\BCi}{{\bfm{\cal i}}}
\newcommand{\BCj}{{\bfm{\cal j}}}
\newcommand{\BCk}{{\bfm{\cal k}}}
\newcommand{\BCl}{{\bfm{\cal l}}}
\newcommand{\BCm}{{\bfm{\cal m}}}
\newcommand{\BCn}{{\bfm{\cal n}}}
\newcommand{\BCo}{{\bfm{\cal o}}}
\newcommand{\BCp}{{\bfm{\cal p}}}
\newcommand{\BCq}{{\bfm{\cal q}}}
\newcommand{\BCr}{{\bfm{\cal r}}}
\newcommand{\BCs}{{\bfm{\cal s}}}
\newcommand{\BCt}{{\bfm{\cal t}}}
\newcommand{\BCu}{{\bfm{\cal u}}}
\newcommand{\BCv}{{\bfm{\cal v}}}
\newcommand{\BCx}{{\bfm{\cal x}}}
\newcommand{\BCy}{{\bfm{\cal y}}}
\newcommand{\BCz}{{\bfm{\cal z}}}
\newcommand{\BCA}{{\bfm{\cal A}}}
\newcommand{\BCB}{{\bfm{\cal B}}}
\newcommand{\BCC}{{\bfm{\cal C}}}
\newcommand{\BCD}{{\bfm{\cal D}}}
\newcommand{\BCE}{{\bfm{\cal E}}}
\newcommand{\BCF}{{\bfm{\cal F}}}
\newcommand{\BCG}{{\bfm{\cal G}}}
\newcommand{\BCH}{{\bfm{\cal H}}}
\newcommand{\BCI}{{\bfm{\cal I}}}
\newcommand{\BCJ}{{\bfm{\cal J}}}
\newcommand{\BCK}{{\bfm{\cal K}}}
\newcommand{\BCL}{{\bfm{\cal L}}}
\newcommand{\BCM}{{\bfm{\cal M}}}
\newcommand{\BCN}{{\bfm{\cal N}}}
\newcommand{\BCO}{{\bfm{\cal O}}}
\newcommand{\BCP}{{\bfm{\cal P}}}
\newcommand{\BCQ}{{\bfm{\cal Q}}}
\newcommand{\BCR}{{\bfm{\cal R}}}
\newcommand{\BCS}{{\bfm{\cal S}}}
\newcommand{\BCT}{{\bfm{\cal T}}}
\newcommand{\BCU}{{\bfm{\cal U}}}
\newcommand{\BCV}{{\bfm{\cal V}}}
\newcommand{\BCW}{{\bfm{\cal W}}}
\newcommand{\BCX}{{\bfm{\cal X}}}
\newcommand{\BCY}{{\bfm{\cal Y}}}
\newcommand{\BCZ}{{\bfm{\cal Z}}}


\def\ii{{\rm i}}
\def\dd{{\rm d}}
\def\Im{{\it Im}}
\def\Re{{\it Re}}
\def\ca{{\cal A}}
\def\ct{{\cal T}}
\def\Ba{{\bf a}}
\def\Bb{{\bf b}}
\def\Bc{{\bf c}}
\def\Bd{{\bf d}}
\def\Be{{\bf e}}
\def\Bf{{\bf f}}
\def\Bg{{\bf g}}
\def\Bh{{\bf h}}
\def\Bi{{\bf i}}
\def\Bj{{\bf j}}
\def\Bk{{\bf k}}
\def\Bl{{\bf l}}
\def\Bm{{\bf m}}
\def\Bn{{\bf n}}
\def\Bo{{\bf o}}
\def\Bp{{\bf p}}
\def\Bq{{\bf q}}
\def\Br{{\bf r}}
\def\Bs{{\bf s}}
\def\Bt{{\bf t}}
\def\Bu{{\bf u}}
\def\Bv{{\bf v}}
\def\Bw{{\bf w}}
\def\Bx{{\bf x}}
\def\By{{\bf y}}
\def\Bz{{\bf z}}
\def\BA{{\bf A}}
\def\BB{{\bf B}}
\def\BC{{\bf C}}
\def\BD{{\bf D}}
\def\BE{{\bf E}}
\def\BF{{\bf F}}
\def\BG{{\bf G}}
\def\BH{{\bf H}}
\def\BI{{\bf I}}
\def\BJ{{\bf J}}
\def\BK{{\bf K}}
\def\BL{{\bf L}}
\def\BM{{\bf M}}
\def\BN{{\bf N}}
\def\BO{{\bf O}}
\def\BP{{\bf P}}
\def\BQ{{\bf Q}}
\def\BR{{\bf R}}
\def\BS{{\bf S}}
\def\BT{{\bf T}}
\def\BU{{\bf U}}
\def\BV{{\bf V}}
\def\BW{{\bf W}}
\def\BX{{\bf X}}
\def\BY{{\bf Y}}
\def\BZ{{\bf Z}}

\def\half{{\scriptstyle{1\over 2}}}
\newcommand{\eps}{\varepsilon}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\overliner}{\begin{eqnarray}}
\newcommand{\earr}{\end{eqnarray}}
\newcommand{\beqn}{\begin{equation*}}
\newcommand{\eeqn}{\end{equation*}}
\newcommand{\overlinern}{\begin{eqnarray*}}
\newcommand{\earrn}{\end{eqnarray*}}
\newcommand{\prt}{\partial}
\newcommand{\sg}{\sigma}
\newcommand{\fr}{\frac}
\newcommand{\kap}{\varkappa}
%\newcommand{\diag}{\mbox{diag}}
\newcommand{\sign}{\mbox{sign}}
\def\l{\label}

%Definitions: journals
\def\AMPA{ Ann. Mat. Pura Appl.}
\def\AMR{ Appl. Mech. Rev.}
\def\AMS{ Acta. Mech. Sin.}
\def\ARMA{ Arch. Rat. Mech. Anal.}
\def\ASCEEM{ ASCE J. Eng. Mech.}
\def\AAM{Adv. Appl. Mech.}
\def\APL{ Appl. Phys. Letters}
\def\CMAME { Comput. Meth. Appl. Mech. Engrg.}
\def\CS { Comput. Struct.}
\def\CRAS{ C. R. Acad. Sci., Paris}
\def\EFM{ Eng. Fract. Mech.}
\def\EJMA{ Eur. J. Mech. A/Solids}
\def\IJES{ Int. J. Eng. Sci.}
\def\IJMS{ Int. J. Mech. Sci.}
\def\IJNAMG{ Int. J. Numer. Anal. Meth. Geomech.}
\def\IJP{ Int. J. Plasticity}
\def\IJSS{ Int. J. Solids Struct.}
\def\IMA{ IMA J. Appl. Math.}
\def\IngA{ Ing. Archiv}
\def\INTERFACE{ J. R. Soc. Interface}
\def\IP{ Inverse Probl.}
\def\JAM{ J. Appl. Mech.}
\def\JAP{ J. Appl. Phys.}
\def\JE{ J. Elasticity}
\def\JEM{ J. Eng. Math.}
\def\JM{ J. de M\'ecanique}
\def\JMP{ J. Math. Phys.}
\def\JMPS{ J. Mech. Phys. Solids}
\def\JOSA{ J. Opt. Soc. Am. A}
\def\JOpt{ J. Opt.}
\def\JPD{ J. Phys. D: Appl. Phys.}
\def\MA{ Macromolecules}
\def\MMS{ Math. Mech. Solids}
\def\MOM{ Mech. Materials}
\def\MRL{ Math. Res. Lett.}
\def\MRSSP{ Mat. Res. Soc. Symp. Proc.}
\def\MTT{ Mekh. Tverd. Tela.}
\def\MPCPS{ Math. Proc. Cambridge Phil. Soc.}
\def\NAT{ Nature}
\def\NJP{ New J. Phys.}
\def\PRA{ Phys. Rev. B}
\def\PRB{ Phys. Rev. B}
\def\PRL{ Phys. Rev. Lett.}
\def\PRSLA{ Proc. R. Soc. Lond. A}
\def\QAM{ Quart. Appl. Math.}
\def\QJMAM{ Quart. J. Mech. Appl. Math.}
\def\RPP{ Rep. Prog. Phys.}
\def\RAN{ Rend. Acc. Naz.}
\def\RCT{ Rubb. Chem. Technol.}


